MobileConvRec: A Conversational Dataset for Mobile Apps Recommendations

Existing recommendation systems have focused on two paradigms: 1- historical user-item interaction-based recommendations and 2- conversational recommendations. Conversational recommendation systems facilitate natural language dialogues between users and the system, allowing the system to solicit users' explicit needs while enabling users to inquire about recommendations and provide feedback. Due to substantial advancements in natural language processing, conversational recommendation systems have gained prominence. Existing conversational recommendation datasets have greatly facilitated research in their respective domains. Despite the exponential growth in mobile users and apps in recent years, research in conversational mobile app recommender systems has faced substantial constraints. This limitation can primarily be attributed to the lack of high-quality benchmark datasets specifically tailored for mobile apps. To facilitate research for conversational mobile app recommendations, we introduce MobileConvRec. MobileConvRec simulates conversations by leveraging real user interactions with mobile apps on the Google Play store, originally captured in large-scale mobile app recommendation dataset MobileRec. The proposed conversational recommendation dataset synergizes sequential user-item interactions, which reflect implicit user preferences, with comprehensive multi-turn conversations to effectively grasp explicit user needs. MobileConvRec consists of over 12K multi-turn recommendation-related conversations spanning 45 app categories. Moreover, MobileConvRec presents rich metadata for each app such as permissions data, security and privacy-related information, and binary executables of apps, among others. We demonstrate that MobileConvRec can serve as an excellent testbed for conversational mobile app recommendation through a comparative study of several pre-trained large language models.

==> tables/tbl_bl_results.tex <==
\begin{table*}[h]
\centering
\caption{Performance Analysis of various baselines on {\ourdataset}. 
\label{tbl:perf-analysis}
%We report \textit{Hit@1}, \textit{Hit@5}, \textit{Hit@10}, \textit{Hit@15}, \textit{Hit@20}, \textit{NDCG@5}, \textit{NDCG@10}, \textit{NDCG@15} and \textit{NDCG@20}. 
Baselines belonging to various categories, such as General baselines (e.g. Pop), Sequential baselines (e.g. SASRec, ELECRec, BERT4Rec, HGN, SINE), Session-based baselines (e.g. GRU4Rec GCSAN), Graph Neural Network based baselines (e.g. GCSAN), Transformer based baselines (e.g. LigthSANs).}

\begin{tabular}{c|ccccccccc}
\toprule
\multicolumn{1}{l}{\textbf{Method $\downarrow$ Metric $\rightarrow$}} & \multicolumn{1}{l}{\textbf{Hit@1}} & \multicolumn{1}{l}{\textbf{Hit@5}} & \multicolumn{1}{l}{\textbf{Hit@10}} & \multicolumn{1}{l}{\textbf{Hit@15}} & \multicolumn{1}{l}{\textbf{Hit@20}} & \multicolumn{1}{l}{\textbf{NDCG@5}} & \multicolumn{1}{l}{\textbf{NDCG@10}} & \multicolumn{1}{l}{\textbf{NDCG@15}} & \multicolumn{1}{l}{\textbf{NDCG@20}} \\ \hline
\textbf{Pop}                                & 0.0027                             & 0.0086                             & 0.0151                              & 0.0208                              & 0.0256                              & 0.0056                              & 0.0077                               & 0.0092                               & 0.0103                               \\
\textbf{SASRec}                             & 0.0026                             & 0.0098                             & 0.0181                              & 0.0242                              & 0.0295                              & 0.0061                              & 0.0088                               & 0.0104                               & 0.0117                               \\
\textbf{ElecRec}                            & 0.0020                             & 0.0094                             & 0.0174                              & 0.0237                              & 0.0293                              & 0.0056                              & 0.0082                               & 0.0098                               & 0.0112                               \\
\textbf{Bert4Rec}                           & 0.0024                             & 0.0083                             & 0.014                               & 0.0183                              & 0.0221                              & 0.0054                              & 0.0072                               & 0.0083                               & 0.0092                               \\
\textbf{HGN}                                & 0.0012                             & 0.0054                             & 0.0096                              & 0.0132                              & 0.0165                              & 0.0033                              & 0.0046                               & 0.0056                               & 0.0064                               \\
\textbf{SINE}                               & 0.0022                             & 0.0087                             & 0.0163                              & 0.0228                              & 0.028                               & 0.0054                              & 0.0078                               & 0.0095                               & 0.0107                               \\
\textbf{LightSANs}                          & 0.0024                             & 0.0102                             & 0.0172                              & 0.0227                              & 0.028                               & 0.0062                              & 0.0085                               & 0.0099                               & 0.0112                               \\
\textbf{GRU4Rec}                            & 0.0021                             & 0.0086                             & 0.0153                              & 0.021                               & 0.0261                              & 0.0053                              & 0.0074                               & 0.0089                               & 0.0102                               \\
\textbf{GCSAN}                              & 0.0024                             & 0.0094                             & 0.0161                              & 0.0214                              & 0.0266                              & 0.0059                              & 0.0081                               & 0.0095                               & 0.0107  \\
\bottomrule
\end{tabular}
%\vspace{-5pt}
\end{table*}

==> tables/tbl_bl_results_old.tex <==
\begin{table*}[t]
\par\vspace{20pt}\par
\resizebox{\textwidth}{!}{%

}
\end{table*}

==> tables/tbl_statistics_v0.tex <==
\begin{table*}[t]
\resizebox{\textwidth}{!}{%

\begin{tabular}{cllllllll}
\toprule
\textbf{Datasets}                      & \textbf{Users with \textgreater 4 interactions} & \textbf{Items with \textgreater 19 interactions} & \textbf{Max. interactions from a user} & \textbf{Min. interactions from a user} & \textbf{Avg. \# items interacted by a user} & \textbf{Max. interactions on an item} & \textbf{Min. interactions on an item} & \textbf{Avg. interactions per item} \\ \hline
\multicolumn{1}{c|}{\textbf{Beauty}}   & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{ML-1M}}    & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{Yelp}}     & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{Stream}}   & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{ML-20M}}   & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{Sports}}   & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{LastFM}}   & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{Toys}}     & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{Games}}    & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{Clothing}} & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\ \hline
\textbf{GooglePlay (Ours)}             &                                                 &                                                  &                                        &                                        &                                             &                                       &                                       &           \\    
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/tbl_statistics_v1.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcllllllllll}
\toprule
\multicolumn{1}{c}{\textbf{Datasets}}                                 & \textbf{Beauty} & \multicolumn{1}{c}{\textbf{ML-1M}} & \multicolumn{1}{c}{\textbf{Yelp}} & \multicolumn{1}{c}{\textbf{Stream}} & \multicolumn{1}{c}{\textbf{ML-20M}} & \multicolumn{1}{c}{\textbf{Sports}} & \textbf{LastFM} & \multicolumn{1}{c}{\textbf{Toys}} & \multicolumn{1}{c}{\textbf{Games}} & \multicolumn{1}{c}{\textbf{Clothing}} & \multicolumn{1}{c}{\textbf{MobileRec (Ours)}} \\ \hline
\multicolumn{1}{l|}{\textbf{Total interactions}}  & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &     \multicolumn{1}{c}{\textbf{19297020}}                                          \\
\multicolumn{1}{l|}{\textbf{Users with \textgreater 4 interactions}}  & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &     \multicolumn{1}{c}{\textbf{700111}}                                          \\
\multicolumn{1}{l|}{\textbf{Items with \textgreater 14 interactions}} & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &                 \multicolumn{1}{c}{\textbf{10173}}                               \\
\multicolumn{1}{l|}{\textbf{Max. interactions from a user}}           & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &        \multicolumn{1}{c}{\textbf{256}}                                        \\
\multicolumn{1}{l|}{\textbf{Min. interactions from a user}}           & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &      \multicolumn{1}{c}{\textbf{5}}                                          \\
\multicolumn{1}{l|}{\textbf{Avg. interactions by a user}}      & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &             \multicolumn{1}{c}{\textbf{27.5628}}                                   \\
\multicolumn{1}{l|}{\textbf{Max. interactions on an item}}            & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &                    \multicolumn{1}{c}{\textbf{14345}}                            \\
\multicolumn{1}{l|}{\textbf{Min. interactions on an item}}            & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &            \multicolumn{1}{c}{\textbf{20}}                                    \\
\multicolumn{1}{l|}{\textbf{Avg. interactions per item}}              & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &     \multicolumn{1}{c}{\textbf{1896.8858}}    \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/tbl_statistics_v2.tex <==
\begin{table*}[t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|clllllllll|l}
\toprule
\multicolumn{1}{c|}{\textbf{Datasets}}           & \textbf{Beauty} & \multicolumn{1}{c}{\textbf{ML-1M}} & \multicolumn{1}{c}{\textbf{Yelp}} & \multicolumn{1}{c}{\textbf{Stream}} & \multicolumn{1}{c}{\textbf{ML-20M}} & \multicolumn{1}{c}{\textbf{Sports}} & \textbf{LastFM} & \multicolumn{1}{c}{\textbf{Toys}} & \multicolumn{1}{c}{\textbf{Games}} & \multicolumn{1}{c|}{\textbf{Clothing}} & \multicolumn{1}{c}{\textbf{GooglePlay (Ours)}} \\ \hline
\textbf{Users with \textgreater 4 interactions}  & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\textbf{Items with \textgreater 19 interactions} & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\textbf{Max. interactions from a user}           & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\textbf{Min. interactions from a user}           & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\textbf{Avg. \# items interacted by a user}      & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\textbf{Max. interactions on an item}            & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\textbf{Min. interactions on an item}            & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\textbf{Avg. interactions per item}              & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/tbl_statistics_v3.tex <==
%Comparison of existing recommendation datasets with {\ourdataset}. Latest versions of \textit{Amazon review data, Yelp, ML-25M} has been used for generating these statistics. \textit{Amazon review data} has 29 categories and was released back in $\mathbf{2018}$. \textit{ML-25M} has 25M movie ratings. $\mathbf{162,000}$ users interacted with $\mathbf{62,000}$ movies, resulting in 1 million tag applications. \textit{ML-25M} dataset was released back in 12/2019. \textit{Yelp} is a large-scale business reviews dataset with various versions. we employ \textit{Yelp2022} which is the latest version.
\begin{table*}[t!]
\centering
\caption{{\ourdataset}'s comparison with the latest versions of well-known recommendation datasets in different domains. We used the Amazon Reviews dataset from 2018, Yelp's 2022 version, and the latest release of ML-25M from 12/2019 to produce these statistics.}
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{c}{\textbf{Datasets}}                                       & \textbf{Amazon Reviews} & \textbf{Yelp} & \textbf{ML-25M} & \textbf{MobileRec (Ours)} \\ \hline
\multicolumn{1}{l|}{Total interactions (in millions)}                                     & 233.1               & 6.99       & 25.0        & 19.3                  \\
\multicolumn{1}{l|}{Users with at least five interactions (in millions)}  & 10.6                & 0.29        & 0.16          & 0.70                    \\
\multicolumn{1}{l|}{Items with at least 15 interactions (in thousands)} & 2072                 & 77.58         & 20.59           & 10.17                     \\
\multicolumn{1}{l|}{Maximum number of interactions by a single user}                          & 446                     & 3048          & 32202           & 256                       \\
\multicolumn{1}{l|}{Minimum number of interactions by a single user}                          & 1                       & 1             & 20              & 5                         \\
\multicolumn{1}{l|}{Average number of interactions per user}                            & 5.32                  & 3.52        & 153.81         & 27.56                     \\
\multicolumn{1}{l|}{Maximum number of interactions on a single item}                           & 13,560                   & 7,673          & 81,491           & 14,345                     \\
\multicolumn{1}{l|}{Minimum number of interactions on a single item}                           & 1                       & 5             & 1               & 20                        \\
\multicolumn{1}{l|}{Average number of interactions per item}                             & 15.45                 & 46.49       & 423.39         & 1896.88                   \\ 
\bottomrule
% \multicolumn{4}{l}{
%       $^\ast$ This table refers to the latest version of \textit{Amazon review data} released in 2018 
%          }
% \multicolumn{4}{l}{
%       $^\dagger$ \textit{Yelp2022} is the latest release of the dataset.}
\end{tabular}
\vspace{-10pt}
\label{tab:compare-rec-datasets}
\end{table*}
